Some Models and Tools for Open Systems

In computer science, there is a distinction between closed systems, whose behavior is totally determined in advance, and open systems, that are systems maintaining a constant interaction with an unspecified environment. Closed systems are naturally modeled by transitions systems. Open systems have been modeled in various ways, including process algebras, I/O automata, ``modules'', and interfaces. Games provide a uniform setting in which all these models can be cast and compared. In this paper, we discuss the features and costs related to the game-based approach to open systems, referring to some of the existing models. Finally, we describe a new model of interface, called sociable interface, which is geared towards easier specification, improved reusability of models, and efficient symbolic implementation.

==> intro-old.tex <==
\section{Introduction}

In computer system design, there is a distinction between {\em closed}
and {\em open} system. A closed system is a system whose behaviors is
totally determined by the state of the system, while an open system is
a system that interacts with its environment and whose behavior
depends on it.

There exists many techniques and tools for verifying closed
systems. Among them, one can find the well known model checking
technique that has been implemented in tools such as
\cite{spin,smv,lash,fast}, as well as other techniques based on
abstraction \cite{grenoble}, or logic formalism and invariant
computation \cite{harvey}.

While the closed system model is very well suited for specifying and
verifying properties of components whose behavior is totally known in
advance (mutual exclusion algorithms, ...), it cannot be use to
express interaction between a component and its possibly unknown
environment. Being able to verify systems whose behavior depends of an
unknown environment is clearly a crucial point that allow a modular
approach to the verification of very complex systems. In this paper,
we focus on the design and the verification of open systems.

One of the very first automata model that have been introduced to
design open systems {\footnote{and closed systems}} is the one of I/O
automata introduced by Lynch and Tuttle in \cite{}. In this framework,
a component is represented by a finite-state automaton whose
transitions are labeled by actions. Among those actions, one
distinguish output and internal actions that reflect the behavior of
the component, and input actions that reflect the one of the
environment. A main particularity of I/O automata is that they are
input-enable everywhere, which means that at any moment the component
must be receptive to environment's behavior.

The I/O automata model has been implemented in various tools such as
\cite{}, or \cite{} and has allowed the verification of very complex
open systems \cite{}. 

One of the main drawback of the approach of \cite{} is that because of
the input-enabled everywhere principle, it is difficult to encode
restrictions on the order of method calls, and on the types of return
values and exceptions.

In a recent series of works \cite{}, de Alfaro et All have introduced
interface models. Basically, Interface models captures the temporal
I/O behavior of a component by an automaton. While this is not the
first automata-based formalism for modeling open systems, the
interface models approach is slightly different from approach closed
to the I/O automata model.

Interface models are in a certain sense I/O automata. However, unlike
I/O automata, which at every state must be receptive towards every
possible input action, interface models can consider some input action
to be illegal in a given state. This approach is called the {\em
optimistic approach}, i.e. the approach in where one expresses the
assumption that the environment never generates these inputs. 

The optimistic approach clearly influence the way in where the
components talk together. If two interface models are composed, the
result can contains error states, in where one of the interface wants
to issue an output action that cannot be catch by an input action of
the other interface. In opposition to the standard approach that would
consider the composition to be bad, the interface model approach
follow again an optimistic approach that consists in considering that
expecting that the environment can stay away from all error
states. The existence of such an environment indicates that the two
interfaces are compatible.

An interface is naturally modeled as a game between the players Output
and Input. An interface is considered to be ``well-formed'' meaning
that there exists at least one environment that satisfies its input
assumptions iff the Input player has a winning strategy in the game,
i.e. the environment can meet all input assumptions. In this game
approach, two interface models are compatible if there is a way for
the input player, who chooses the inputs of the composite interface to
avoid all bad states.

Existing interface models are divided into interface automata
\cite{FSE01-IA,IA-Marktoberdorf04} and interface modules
\cite{EMSOFT01,CAV02-IM} that are based on either actions, or
variables, but not both.

Recently we have introduce an interface model that can communicate via
both actions and variables, and that provide one-to-one, many-to-one,
one-to-many, and many-to-many communication and synchronization.  We
show that this rich communication semantics can be achieved by
combining a small number of basic concepts, thanks to the expressive
power of interface models. This leads to an uniform, and conceptually
simple, communication model. We call this model \cu{sociable
interfaces,} underlining the ease with which these interfaces can be
composed into models of design. While sociable interfaces do not
break new ground in the conceptual theory of interface models, we hope
that they constitute a useful step towards a practical,
interface-based design methodology.  

{\paragraph{Outline}} 

The rest of the paper is divided into two sections. In Section \ref{sec-literature},
we make a short survey of existing works and tools for specifying and
verifying open systems. In section \ref{sec-sociable}, 
we present a novel type of interfaces called \emph{Sociable Interfaces}.


==> printer-nak-frocos.tex <==
\begin{verbatim}
var busy: bool;    // global variable indicating a printer busy 
var size: [0..10]; // size of the print job
var user: [0..5];  // user who requested the job 

module Printer:
  output ack   { busy & size < 5 ==> not busy'; } // accept if size < 5
                               // ack? is not allowed

  output nack  { busy & size > 4 ==> not busy'; } // reject if size > 4
                               // nack? is not allowed

  input  print { global: not busy ==> busy'; }
endmodule

module User1:
  var s: [0..1];
  stateless size, user; 

  output print { s = 0 & not busy ==> 
                                  s' = 1 & user' = 1 & nondet size'; }
  input  print { }  // print? is allowed and ignored 

  input  ack   { local: s = 1 ==> s' := 0; 
                  else  s = 0 ==> ;        }  // ignore ack? when s=0 

  input  nack  { local: s = 1 ==> s' := 0; 
                  else  s = 0 ==> ;        }  // ignore nack? when s=0 
endmodule

module User2:
  var s: [0..1];
  stateless size, user; 

  output print { s = 0 & not busy ==> 
                                  s' = 1 & user' = 2 & nondet size'; }
  input  print { }  // print? is allowed and ignored 

  input  ack   { local: s = 1 ==> s' := 0; 
                 else   s = 0 ==> ;        }  // ignore ack? when s=0 

  input  nack  { local: s = 1 ==> s' := 0; 
                 else   s = 0 ==> ;        }  // ignore nack? when s=0 
endmodule
\end{verbatim}

